Parabolic Multiplicative Affine Springer Fibers

We introduce parabolic multiplicative affine Springer fibers, which resemble the admissible union of affine Deligne Lusztig varieties in the affine flag variety. We also study their global counterparts called parabolic multiplicative Hitchin fibers. Their associated fibration is a global analogue of the Grothendieck simultaneous resolution for monoids. Using this fibration, we show that the parabolic multiplicative affine Springer fibers are equidimensional and find their dimension.

==> bib.tex <==
@MISC{SP,
    AUTHOR = "Authors, The Stacks Project",
    TITLE = "Stacks Project",
    URL = "https://stacks.math.columbia.edu/"
}

@article{Vin95,
title = {On Reductive Algebraic Semigroups},
journal = {Lie groups and Lie algebras: E. B. Dynkin's Seminar},
volume = {},
number = {},
pages = {145-182},
year = {1995},
issn = {},
doi = {MR1364458},
url = {},
author = {E.B. Vinberg},
}
@article{G10,
     author = {Pezzini, Guido},
     title = {Lectures on spherical and wonderful varieties},
     booktitle = {Actions hamiltoniennes~: invariants et classification. 6 {\textendash} 10 avril 2009},
     author = {Collectif},
     series = {Les cours du CIRM},
     pages = {33--53},
     publisher = {CIRM},
     number = {1},
     year = {2010},
     doi = {10.5802/ccirm.3},
     language = {en},
     url = {http://www.numdam.org/articles/10.5802/ccirm.3/}
}

@inproceedings{BK04,
  title={Frobenius splitting methods in geometry and representation theory},
  author={Michel Brion and Shrawan Kumar},
  year={2004},
  url={https://api.semanticscholar.org/CorpusID:117008164}
}

@article{Ren90,
  title={Linear algebraic monoids},
  author={Lex E. Renner},
  journal={Semigroup Forum},
  year={1990},
  volume={40},
  pages={251-254},
  url={https://api.semanticscholar.org/CorpusID:117914466}
}

@article{Put82,
 ISSN = {00029947},
 URL = {http://www.jstor.org/stable/1998722},
 abstract = {},
 author = {Mohan S. Putcha},
 journal = {Transactions of the American Mathematical Society},
 number = {2},
 pages = {693--709},
 publisher = {American Mathematical Society},
 title = {Connected Algebraic Monoids},
 urldate = {2024-01-10},
 volume = {272},
 year = {1982}
}

@article{Chi22, title={Geometry of Kottwitz-Viehmann Varieties}, volume={21}, DOI={10.1017/S1474748019000604}, number={1}, journal={Journal of the Institute of Mathematics of Jussieu}, publisher={Cambridge University Press}, author={Chi, Jingren}, year={2022}, pages={1–65}}

@article{Yun11,
title = {Global Springer theory},
journal = {Advances in Mathematics},
volume = {228},
number = {1},
pages = {266-328},
year = {2011},
issn = {0001-8708},
doi = {https://doi.org/10.1016/j.aim.2011.05.012},
url = {https://www.sciencedirect.com/science/article/pii/S0001870811001629},
author = {Zhiwei Yun},
keywords = {Hitchin fibration, Springer representations, Double affine Hecke algebra},
abstract = {We generalize Springer representations to the context of groups over a global function field. The global counterpart of the Grothendieck simultaneous resolution is the parabolic Hitchin fibration. We construct an action of the graded double affine Hecke algebra (DAHA) on the direct image complex of the parabolic Hitchin fibration. In particular, we get representations of the degenerate graded DAHA on the cohomology of parabolic Hitchin fibers, providing the first step towards a global Springer theory.}
}

@article{Ngo08,
     author = {Ng\^o, Bao Ch\^au},
     title = {Le lemme fondamental pour les alg\`ebres de {Lie}},
     journal = {Publications Math\'ematiques de l'IH\'ES},
     pages = {1--169},
     publisher = {Springer-Verlag},
     volume = {111},
     year = {2010},
     doi = {10.1007/s10240-010-0026-7},
     mrnumber = {2653248},
     zbl = {1200.22011},
     language = {fr},
     url = {http://www.numdam.org/articles/10.1007/s10240-010-0026-7/}
}
@article{Lus81,
title = {Green polynomials and singularities of unipotent classes},
journal = {Advances in Mathematics},
volume = {42},
number = {2},
pages = {169-178},
year = {1981},
issn = {0001-8708},
doi = {https://doi.org/10.1016/0001-8708(81)90038-4},
url = {https://www.sciencedirect.com/science/article/pii/0001870881900384},
author = {G Lusztig}
}

@misc{Wang23,
      title={Multiplicative Hitchin Fibration and Fundamental Lemma}, 
      author={X. Griffin Wang},
      year={2024},
      eprint={2402.19331},
      archivePrefix={arXiv},
      primaryClass={math.AG}
}

@misc{FN11,
      title={Geometrization of Trace Formulas}, 
      author={Edward Frenkel and Bao Chau Ngo},
      year={2011},
      eprint={1004.5323},
      archivePrefix={arXiv},
      primaryClass={math.RT}
}

@article{GHKR06,
     author = {G\"ortz, Ulrich and Haines, Thomas J. and Kottwitz, Robert E. and Reuman, Daniel C.},
     title = {Dimensions of some affine {Deligne-Lusztig} varieties},
     journal = {Annales scientifiques de l'\'Ecole Normale Sup\'erieure},
     pages = {467--511},
     publisher = {Elsevier},
     volume = {Ser. 4, 39},
     number = {3},
     year = {2006},
     doi = {10.1016/j.ansens.2005.12.004},
     zbl = {1108.14035},
     language = {en},
     url = {http://www.numdam.org/articles/10.1016/j.ansens.2005.12.004/}
}

@incollection{Rap05,
     author = {Rapoport, Michael},
     title = {A guide to the reduction modulo $p$ of {Shimura} varieties},
     booktitle = {Formes automorphes (I) - Actes du semestre du centre \'Emile Borel, printemps 2000},
     editor = {Tilouine Jacques and Carayol Henri and Harris Michael and Vign\'eras Marie-France},
     series = {Ast\'erisque},
     publisher = {Soci\'et\'e math\'ematique de France},
     number = {298},
     year = {2005},
     zbl = {1084.11029},
     mrnumber = {2141705},
     language = {en},
     url = {http://www.numdam.org/item/AST_2005__298__271_0/}
}

@ARTICLE{He14,
       author = {{He}, Xuhua},
        title = "{Kottwitz-Rapoport conjecture on unions of affine Deligne-Lusztig varieties}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Algebraic Geometry, Mathematics - Number Theory, Mathematics - Representation Theory},
         year = 2014,
        month = aug,
          eid = {arXiv:1408.5838},
        pages = {arXiv:1408.5838},
          doi = {10.48550/arXiv.1408.5838},
archivePrefix = {arXiv},
       eprint = {1408.5838},
 primaryClass = {math.AG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1408.5838H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Zho19,
      title={Convex Polytopes for the Central Degeneration of the Affine Grassmannian}, 
      author={Qiao Zhou},
      year={2019},
      eprint={1604.08641},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/1604.08641}, 
}

@article{HY21,
author = {He, Xuhua and Yu, Qingchao},
year = {2021},
month = {04},
pages = {1-19},
title = {Dimension formula for the affine Deligne–Lusztig variety $X(\mu, b)$},
volume = {379},
journal = {Mathematische Annalen},
doi = {10.1007/s00208-020-02102-5}
}


@misc{He23,
      title={On affine Lusztig varieties}, 
      author={Xuhua He},
      year={2023},
      note={arXiv:2302.03203},
      archivePrefix={arXiv},
      primaryClass={math.RT}
}

@misc{Lus10,
      title={From conjugacy classes in the Weyl group to unipotent classes}, 
      author={G. Lusztig},
      year={2010},
      note={arXiv:1003.0412},
      archivePrefix={arXiv},
      primaryClass={math.RT}
}

@article{Zhu14,
 ISSN = {0003486X},
 URL = {http://www.jstor.org/stable/24522918},
 abstract = {We prove the (generalized) coherence conjecture proposed by Pappas and Rapoport. As a corollary, one of their theorems, which describes the geometry of the special fibers of the local models for ramified unitary groups, holds unconditionally. Our proof is based on the study of the geometry (in particular, certain line bundles and l-adic sheaves) of the global Schubert varieties, which are the equal characteristic counterparts of the local models.},
 author = {Xinwen Zhu},
 journal = {Annals of Mathematics},
 number = {1},
 pages = {1--85},
 publisher = {Annals of Mathematics},
 title = {On the coherence conjecture of Pappas and Rapoport},
 urldate = {2023-10-27},
 volume = {180},
 year = {2014}
}
@misc{HR19,
      title={Normality and Cohen-Macaulayness of parahoric local models}, 
      author={Thomas J. Haines and Timo Richarz},
      year={2019},
      eprint={1903.10585},
      archivePrefix={arXiv},
      primaryClass={math.AG}
}
@misc{zhu16,
      title={An introduction to affine Grassmannians and the geometric Satake equivalence}, 
      author={Xinwen Zhu},
      year={2016},
      eprint={1603.05593},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/1603.05593}, 
}
@article{PZ13, 
title={Local models of Shimura varieties and a conjecture of Kottwitz}, volume={194}, ISSN={0020-9910}, DOI={10.1007/s00222-012-0442-z}, abstractNote={We give a group theoretic definition of "local models" as sought after in the theory of Shimura varieties. These are projective schemes over the integers of a p-adic local field that are expected to model the singularities of integral models of Shimura varieties with parahoric level structure. Our local models are certain mixed characteristic degenerations of Grassmannian varieties; they are obtained by extending constructions of Beilinson, Drinfeld, Gaitsgory and the second-named author to mixed characteristics and to the case of general (tamely ramified) reductive groups. We study the singularities of local models and hence also of the corresponding integral models of Shimura varieties. In particular, we study the monodromy (inertia) action and show a commutativity property for the sheaves of nearby cycles. As a result, we prove a conjecture of Kottwitz which asserts that the semi-simple trace of Frobenius on the nearby cycles gives a function which is central in the parahoric Hecke algebra.}, note={Funding by NSF}, number={1}, journal={Inventiones Mathematicae}, publisher={Springer}, author={Pappas, G. and Zhu, X.}, year={2013}, month={Oct}, pages={147–254} }

@article{BC18,
author = {Bouthier, Alexis and Chi, Jingren},
year = {2018},
month = {12},
pages = {},
title = {Correction to: Dimension des fibres de Springer Affines pour les groupes},
volume = {23},
journal = {Transformation Groups},
doi = {10.1007/s00031-018-9496-3}
}

@incollection{Kat79,
     author = {Katz, Nicholas M.},
     title = {Slope filtration of $f$-crystals},
     booktitle = {Journ\'ees de G\'eom\'etrie Alg\'ebrique de Rennes - (Juillet 1978) (I) : Groupe formels, repr\'esentations galoisiennes et cohomologie des vari\'et\'es de caract\'eristique positive},
     series = {Ast\'erisque},
     pages = {113--163},
     publisher = {Soci\'et\'e math\'ematique de France},
     number = {63},
     year = {1979},
     mrnumber = {563463},
     zbl = {0426.14007},
     language = {en},
     url = {http://www.numdam.org/item/AST_1979__63__113_0/}
}

@misc{HM03,
      title={Elliptic Sklyanin integrable systems for arbitrary reductive groups}, 
      author={Jacques Hurtubise and Eyal Markman},
      year={2003},
      eprint={math/0203031},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/math/0203031}, 
}

@misc{KV10,
      title={Generalized affine Springer fibers}, 
      author={Robert Kottwitz and Eva Viehmann},
      year={2010},
      eprint={arXiv:1003.2135},
      primaryClass={math.RT}
}

@article{Yun12, title={Langlands duality and global Springer theory}, volume={148}, DOI={10.1112/S0010437X11007433}, number={3}, journal={Compositio Mathematica}, publisher={London Mathematical Society}, author={Yun, Zhiwei}, year={2012}, pages={835–867}}

@article{KL88,
  title={Fixed point varieties on affine flag manifolds},
  author={David Kazhdan and George Lusztig},
  journal={Israel Journal of Mathematics},
  year={1988},
  volume={62},
  pages={129-168},
  url={https://api.semanticscholar.org/CorpusID:120433187}
}

@article{Bez96,
  title={The dimension of the fixed point set on affine flag manifolds},
  author={Roman Bezrukavnikov},
  journal={Mathematical Research Letters},
  year={1996},
  volume={3},
  pages={185-189},
  url={https://api.semanticscholar.org/CorpusID:10172409}
}

@article{GHKR10,
author = {Goertz, Ulrich and Haines, Thomas and Kottwitz, Robert and Reuman, Daniel},
year = {2010},
month = {09},
pages = {1339-1382},
title = {Affine Deligne-Lusztig varieties in affine flag varieties},
volume = {146},
journal = {Compositio Mathematica},
doi = {10.1112/S0010437X10004823}
}

@article{Bou12,
  title={Dimesion des fibres de Springer Affines pour les groupes},
  author={Alexis Bouthier},
  journal={Transformation Groups},
  year={2012},
  volume={20},
  pages={615-663},
  url={https://api.semanticscholar.org/CorpusID:53121906}
}

@article{Hit87,
author = {Nigel Hitchin},
title = {{Stable bundles and integrable systems}},
volume = {54},
journal = {Duke Mathematical Journal},
number = {1},
publisher = {Duke University Press},
pages = {91 -- 114},
year = {1987},
doi = {10.1215/S0012-7094-87-05408-1},
URL = {https://doi.org/10.1215/S0012-7094-87-05408-1}
}

@article{Bou14,
  title={La fibration de Hitchin-Frenkel-Ngo et son complexe d'intersection},
  author={Alexis Bouthier},
  journal={arXiv: Group Theory},
  year={2014},
  url={https://api.semanticscholar.org/CorpusID:55697888}
}

@article{Ong23,
  title={Multiplicative Global Springer Theory},
  author={Marielle Ong},
  journal={Ph.D. thesis, to be submitted},
  year={2024},
  url={}
}

@article{EP19,
	doi = {10.1007/s00029-019-0510-y},
  
	url = {https://doi.org/10.1007%2Fs00029-019-0510-y},
  
	year = 2019,
	month = {oct},
  
	publisher = {Springer Science and Business Media {LLC}
},
  
	volume = {25},
  
	number = {4},
  
	author = {Chris Elliott and Vasily Pestun},
  
	title = {Multiplicative Hitchin systems and supersymmetric gauge theory},
  
	journal = {Selecta Mathematica}
}

@misc{Ric15,
      title={Kostant section, universal centralizer, and a modular derived Satake equivalence}, 
      author={Simon Riche},
      year={2015},
      note={arXiv:1411.3112},
      archivePrefix={arXiv},
      primaryClass={math.RT}
}

@article{Hai01,
author = {Thomas J. Haines},
title = {{Test functions for Shimura varieties: the Drinfeld case}},
volume = {106},
journal = {Duke Mathematical Journal},
number = {1},
publisher = {Duke University Press},
pages = {19 -- 40},
year = {2001},
doi = {10.1215/S0012-7094-01-10612-1},
URL = {https://doi.org/10.1215/S0012-7094-01-10612-1}
}

@misc{BV24,
      title={Affine Springer fibers and depth zero L-packets}, 
      author={Roman Bezrukavnikov and Yakov Varshavsky},
      year={2024},
      note={arXiv:2104.13123},
      archivePrefix={arXiv},
      primaryClass={math.RT}
}

@book{Ren10,
  title={Linear Algebraic Monoids},
  author={Renner, L.E.},
  isbn={9783642063497},
  series={Encyclopaedia of Mathematical Sciences},
  url={https://books.google.com/books?id=N0iAcgAACAAJ},
  year={2010},
  publisher={Springer Berlin Heidelberg}
}


@Inbook{Spal82,
author="Spaltenstein, Nicolas",
title="Classes unipotentes",
bookTitle="Classes Unipotentes et Sous-groupes de Borel",
year="1982",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="8--41",
isbn="978-3-540-39335-1",
doi="10.1007/BFb0096304",
url="https://doi.org/10.1007/BFb0096304"
}

@article{BNS16,
 ISSN = {00029327, 10806377},
 URL = {http://www.jstor.org/stable/24736217},
 author = {A. Bouthier and B. C. Ngô and Y. Sakellaridis},
 journal = {American Journal of Mathematics},
 number = {1},
 pages = {81--108},
 publisher = {The Johns Hopkins University Press},
 title = {On the formal arc space of a reductive monoid},
 urldate = {2024-03-25},
 volume = {138},
 year = {2016}
}
@inproceedings{Sad22,
  title={On the dimension of some union of affine Deligne-Lusztig varieties},
  author={Arghya Sadhukhan},
  year={2022},
  url={https://api.semanticscholar.org/CorpusID:254591371}
}


@book{BLR12,
  title={N{\'e}ron Models},
  author={Bosch, S. and L{\"u}tkebohmert, W. and Raynaud, M.},
  isbn={9783642514388},
  series={Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge / A Series of Modern Surveys in Mathematics},
  url={https://books.google.com/books?id=BNfnCAAAQBAJ},
  year={2012},
  publisher={Springer Berlin Heidelberg}
}

@article{Cass21,
   title={Central elements in affine modpHecke algebras via perverse -sheaves},
   volume={157},
   ISSN={1570-5846},
   url={http://dx.doi.org/10.1112/S0010437X2100751X},
   DOI={10.1112/s0010437x2100751x},
   number={10},
   journal={Compositio Mathematica},
   publisher={Wiley},
   author={Cass, Robert},
   year={2021},
   month=sep, pages={2215–2241} }

@book{Ste74,
  title={Conjugacy Classes in Algebraic Groups},
  author={Steinberg, R.},
  isbn={9783540066576},
  lccn={lc73021212},
  series={Lecture notes in mathematics},
  url={https://books.google.com/books?id=WfxUAAAAYAAJ},
  year={1974},
  publisher={Springer-Verlag}
}
@book{Can14,
  title={Algebraic Monoids, Group Embeddings, and Algebraic Combinatorics},
  author={Can, M. and Li, Z. and Steinberg, B. and Wang, Q.},
  isbn={9781493909384},
  series={Fields Institute Communications},
  url={https://books.google.com/books?id=R7suBAAAQBAJ},
  year={2014},
  publisher={Springer New York}
}

@article{Put11,
  title={Root Semigroups in reductive Monoids},
  author={Mohan S. Putcha},
  journal={Int. J. Algebra Comput.},
  year={2011},
  volume={21},
  pages={433-448},
  url={https://api.semanticscholar.org/CorpusID:42702351}
}

@article{Stein65,
author = {Steinberg, Robert},
journal = {Publications Mathématiques de l'IHÉS},
keywords = {group theory},
language = {eng},
pages = {49-80},
publisher = {Institut des Hautes Études Scientifiques},
title = {Regular elements of semi-simple algebraic groups},
url = {http://eudml.org/doc/103853},
volume = {25},
year = {1965},
}

@article{Spalt76,
title = {The Fixed Point Set of a Unipotent Transformation on the Flag Manifold},
journal = {Indagationes Mathematicae (Proceedings)},
volume = {79},
number = {5},
pages = {452-456},
year = {1976},
issn = {1385-7258},
doi = {https://doi.org/10.1016/S1385-7258(76)80008-X},
url = {https://www.sciencedirect.com/science/article/pii/S138572587680008X},
author = {N. Spaltenstein}
}

@misc{Hai04,
      title={Introduction to Shimura varieties with bad reduction of parahoric type}, 
      author={Thomas J. Haines},
      year={2004},
      eprint={math/0409482},
      archivePrefix={arXiv},
      primaryClass={math.AG}
}

@article{Lus84,
author = {Lusztig, G.},
journal = {Inventiones mathematicae},
keywords = {reductive connected algebraic group; unipotent element; irreducible components; variety of Borel subgroups; irreducible representations; permutation representation; Levi decomposition; irreducible cuspidal representation; Coxeter group; generalized Springer correspondence; special orthogonal groups; intersection cohomology},
pages = {205-272},
title = {Intersection cohomology complexes on a reductive group.},
url = {http://eudml.org/doc/143096},
volume = {75},
year = {1984},
}



@article{Lus96,
  title={Affine weyl groups and conjugacy classes in Weyl groups},
  author={George Lusztig},
  journal={Transformation Groups},
  year={1996},
  volume={1},
  pages={83-97},
  url={https://api.semanticscholar.org/CorpusID:121386740}
}

@article{GGP24,
   title={Multiplicative Higgs bundles and involutions},
   volume={451},
   ISSN={0001-8708},
   url={http://dx.doi.org/10.1016/j.aim.2024.109789},
   DOI={10.1016/j.aim.2024.109789},
   journal={Advances in Mathematics},
   publisher={Elsevier BV},
   author={Gallego, Guillermo and García-Prada, Oscar},
   year={2024},
   month=aug, pages={109789} }

@misc{CH09,
      title={Singular Hermitian-Einstein monopoles on the product of a circle and a Riemann surface}, 
      author={Benoit Charbonneau and Jacques Hurtubise},
      year={2009},
      eprint={0812.0221},
      archivePrefix={arXiv},
      primaryClass={math.DG},
      url={https://arxiv.org/abs/0812.0221}, 
}

@misc{Smi15,
      title={Singular $G$-monopoles on $S^1\times \Sigma$}, 
      author={Benjamin H. Smith},
      year={2015},
      eprint={1501.03337},
      archivePrefix={arXiv},
      primaryClass={math.DG},
      url={https://arxiv.org/abs/1501.03337}, 
}

@misc{Yun16,
      title={Lectures on Springer theories and orbital integrals}, 
      author={Zhiwei Yun},
      year={2016},
      eprint={1602.01451},
      archivePrefix={arXiv},
      primaryClass={math.RT},
      url={https://arxiv.org/abs/1602.01451}, 
}
